Improving the Robustness of the Projected Gradient Descent Method for Nonlinear Constrained Optimization Problems in Topology Optimization

The Projected Gradient Descent (PGD) algorithm is a widely used and efficient first-order method for solving constrained optimization problems due to its simplicity and scalability in large design spaces. Building on recent advancements in the PGD algorithm where an inertial step component has been introduced to improve efficiency in solving constrained optimization problems this study introduces two key enhancements to further improve the algorithm's performance and adaptability in large-scale design spaces. First, univariate constraints (such as design variable bounds constraints) are directly incorporated into the projection step via the Schur complement and an improved active set algorithm with bulk constraints manipulation, avoiding issues with min-max clipping. Second, the update step is decomposed relative to the constraint vector space, enabling a post-projection adjustment based on the state of the constraints and an approximation of the Lagrangian, significantly improving the algorithm's robustness for problems with nonlinear constraints. Applied to a topology optimization problem for heat sink design, the proposed PGD algorithm demonstrates performance comparable to or exceeding that of the Method of Moving Asymptotes (MMA), with minimal parameter tuning. These results position the enhanced PGD as a robust tool for complex optimization problems with large variable space, such as topology optimization problems.

==> src/active_set_archive.tex <==
\label{sec::active_set}
The QP problem that arises from Equations \eqref{eq::min_update}, \eqref{eq::eq_constraints_on_update}, and \eqref{eq::ineq_constraints_on_update}, is solved using an active set approach based on the method. Solving these equations gives the optimal projection of $\bm{\tilde{\phi}}^{n+1}$ onto the feasible set $\mathcal{Q}$ using a linearization of the constraint equations $f_j(\bm{\phi})$ around the current iterate $\bm{\phi}^n$. This projection problem, when solved using an active set, can be separated into two sections: the projection and the active set identification. The projection step on a given active set is presented first, followed by the definition of the active set identification algorithm.

The projection on a pre-identified set of constraints in the linearized projection problem involves projecting the point $\bm{\tilde{\phi}}^{n+1}$ onto the intersection of the hyperplanes formed by the active set of linearized constraints to find $\Delta \bm{\phi}^n$. This implies that this iteration treats inequality constraints within the active set as equality constraints. The set of indices of the active constraints is denoted as $J$, and the subspace bound by the constraint part of $J$ is noted $\mathcal{J}$.

The resulting projection of $\bm{\tilde{\phi}}^{n+1}$ onto $\mathcal{Q}$ using the Lagrange multiplier approach is given by:
\begin{align}
    \bm{\phi}^{n+1} &= \bm{\phi}^n - \left(  \Delta\bm{\Tilde{\phi}}^n+ \sum_{j \in J} y_j \dd {f_j(\bm{\phi}^n)}{\bm{\phi}^n}\right),
    \label{eq::updated_point}
\end{align}
where $y_j$ are the Lagrange multipliers associated with the current active set. The Lagrange multipliers are obtained by solving the following matrix system resulting from the linearization of Equations \eqref{eq::eq_constraints_on_update} and \eqref{eq::ineq_constraints_on_update}:
\begin{align}
    A_{{i^*}{j^*}} &= \dd {f_{i^*}(\bm{\phi}^n)}{\bm{\phi}^n} \cdot \dd {f_{j^*}(\bm{\phi}^n)}{\bm{\phi}^n}, \\
    b_{i^*} &= -(a_{i^*} - f_{i^*}(\bm{\phi}^n)) -\dd {f_{i^*}(\bm{\phi}^n)}{\bm{\phi}^n} \cdot   \Delta\bm{\Tilde{\phi}}^n, \\
    \bm{y} &= A^{-1} \bm{b}.
\end{align}

Here, the indices ${i^*}$ and ${j^*}$ refer to the constraints' indices within the active set, not their global indices (\ie the indices of the constraint within Equation \eqref{eq::eq_constraints_function} and \eqref{eq::ineq_constraints_function}). This means that for each component of the vector $\bm{y}$, we must record to which global constraint index it corresponds to. 

In topology optimization problems, it is common to have many univariate constraints in the form of $d \leq \phi_i \leq e$. These constraints are typically maintained using a min--max function clipping \cite{bertsekas2014constrained}. The main advantage of this approach is that the linear problem resulting from the projection of a point onto the intersection of the constraints' hyperplanes remains relatively small since, for most applications, $m \ll k$ in the absence of univariate constraints. However, the clipping approach often results in a loss of optimality in the projection because the Lagrange multipliers associated with other constraints are either adjusted after the projection step to preserve the univariate constraints without considering the optimality of the projection or the Lagrange multipliers are not corrected, leading to none respect of constraints.

To address this issue, the projection step is resolved using a Schur complement approach, which directly incorporates the univariate constraints into the projection step. This method allows for an accurate evaluation of the contribution of univariate constraints to the update vector $\Delta \bm{\phi}$. The active constraints are divided into two blocks: global constraints (\ie those that are not univariate) and univariate constraints. The number of active global constraints is denoted by $m^*$ while the total size of the active constraint set is denoted $\hat{m}$, with $\hat{m} \leq m$. Using this separation, the matrix used to calculate the Lagrange multipliers takes the following form; note that hereafter, for simplicity $f_j(\bm{\phi}^n) \equiv f_j $:

\begin{align}
    M&=
    \begin{bmatrix}
        A & B^t \\
        B & D 
    \end{bmatrix}\label{eq::schur_complement_1} \\
    A_{{i^*}{j^*}} &= \dd {f_{i^*}}{\bm{\phi}^n} \cdot \dd {f_{j^*}}{\bm{\phi}^n} \quad \text{for } {i^*} < m^* \text{ and } {j^*} < m^*\label{eq::schur_complement_2} \\
    B_{({i^*}-m^*){j^*}} &= \frac{d f_{i^*}}{d \phi^n_{\hat{k}}} \dd {f_{j^*}}{\phi^n_{\hat{k}}}  \quad \text{for } {i^*} \geq m^* \text{ and } {j^*} < m^* \label{eq::schur_complement_3}\\
    D_{({i^*}-m^*)({j^*}-m^*)} &= 
    \begin{cases}
        \left(\frac{d f_{i^*}}{d \phi^n_{\hat{k}}}\right)^2, & \text{if } {i^*} = {j^*} \\
        0, & \text{otherwise}
    \end{cases} \quad \text{for } {i^*} \geq m^* \text{ and } {j^*} \geq m^* \label{eq::schur_complement_4}\\
    \bm{b}&=\begin{bmatrix}
        \bm{b_1} \\
        \bm{b_2}
    \end{bmatrix}= 
        \begin{cases}
       -(a_{i^*} - f_{i^*}) - \dd {f_{i^*}}{\bm{\phi}^n} \cdot   \Delta\bm{\Tilde{\phi}}^n, & \text{if } {i^*} < m^* \\
        -(a_{i^*} - f_{i^*}) - \frac{d f_{i^*}}{d \phi^n_{\hat{k}}}  \Delta\Tilde{\phi}^n_{\hat{k}}, & \text{otherwise}
    \end{cases} \label{eq::schur_complement_5} \\
    \bm{y}&=\begin{bmatrix}
        \bm{y_1} \\
        \bm{y_2}
    \end{bmatrix}= {M}^{-1} \bm{b}
    \label{eq::schur_complement_6}
\end{align}

In Equations \eqref{eq::schur_complement_1} to \eqref{eq::schur_complement_6}, the indices $\hat{k}$ refer to the components of $\bm{\phi}^n$ to which the univariate constraints correspond. Here, the block $D$ is a simple diagonal matrix, and in the case of our univariate constraint in the form  $d \leq \phi_i \leq e$, it takes the form of an identity matrix of size $\hat{m}-m^*$. This significantly simplifies the resolution, making the assembly and resolution of this system a much more manageable task using a Schur complement:
\begin{align}
    \bm{y_1} &= (A-BD^{-1} B^t)^{-1} (\bm{b_1}-B^tD^{-1}\bm{b_2}),\\
    \bm{y_2} &= D^{-1}(\bm{b_2}-B\bm{y_1}).
\end{align}
Indeed, since $D$ is diagonal, the resolution only implies the resolution of an $m^*$ by $m^*$ system of linear equations. Note that assembling this matrix system does not require heavy communication in a parallel distributed software architecture since most communication involves distributing the results of vector dot products, which are highly optimized operations. The other necessary operations are all local to each processor. Without the Schur complement, the resolution of the linear system arising in the projection problem would be unpractical for topology optimization problems.


%%% Heavely modified 
To identify the active set of constraints, Wong \cite{wong2011active} proposed an efficient and robust iterative approach, where constraints are added and removed if the Lagrange multipliers are negative. Each sub iteration of the active set definition is indexed by $o$. If some constraints from the active set are removed, the Lagrange multipliers are reevaluated before defining the update. However, the large number of univariate constraints requires bulk manipulation of constraints to be numerically efficient. As such, the algorithm steps are modified to account  for the bulk manipulation of constraints, resulting in the following steps:
\begin{enumerate}
    \item Add all the equality constraints into the initial active constraints set $\mathcal{J}^0$.
    \item Initialize the update vector $\Delta \bm{\phi}^{n,o}$ with $  \Delta\bm{\Tilde{\phi}}^n$ (Equation \eqref{eq::delta_phi_tilde}). 
    \item Update the previous active set $\mathcal{J}^{o-1}$ by adding all the inequality constraints (including univariate constraints) that would be broken along the current update vector $\Delta \bm{\phi}^{n,o}$ to the active set and obtain  $\tilde{\mathcal{J}_{o}}$. This is done by evaluating a linearization of Equation  \eqref{eq::ineq_constraints_on_update}:
    \begin{align}
     f_j-\Delta \bm{\phi}^n \cdot \dd{f_j}{\bm{\phi}^n} \leq a_j \text{ for } j=l+1,l+2, ..,m. 
    \end{align}
    \item Evaluate the size of the active set of constraints. If its size is superior to the size of $\bm{\phi}^n$ (if $\hat{m} > k$), relax the initial guess $\Delta\bm{\Tilde{\phi}}^n$ by a factor $\zeta \in (0,1)$. In practice, this is done by multiplying both $\alpha^n$ and $\beta^n$ by $\zeta$ and reevaluating $\Delta\bm{\Tilde{\phi}}^n$. The value $\zeta =0.5$ was found to be adequate. Return to step 1 with the new initial guess and clear the active set. 
    \item Compute the projection of $\bm{\tilde{\phi}}^{n+1}$ on the
    on the current active set $\tilde{\mathcal{J}}^o$ by solving Equations \eqref{eq::min_update},\eqref{eq::eq_constraints_on_update}, and \eqref{eq::ineq_constraints_on_update}, using Equations \eqref{eq::schur_complement_1} to \eqref{eq::schur_complement_6}. If constraints were added in step 3, go back to step 3 after evaluating the projection on the active set and check for newly broken constraints. Otherwise, continue to step 6.
    \item  Remove inequality constraints within the active set having a negative Lagrange multiplier. This step is split into two phases:
        \begin{itemize}
            \item First, if newly added constraints $(\tilde{\mathcal{J}}^o \setminus \mathcal{J}^{o-1})$ have negative Lagrange multipliers, remove them from the active set and go back to step 5 with the updated active set.
            \item Second, if all new constraints $(\tilde{\mathcal{J}}^o \setminus \mathcal{J}^{o-1})$ have positive Lagrange multipliers, remove all remaining constraints with negative Lagrange multiplier and go back to step 5 with the updated active set.
        \end{itemize}
    If no constraint was removed from the active set, indicating that the KKT criteria on the active set were respected, the active set of the current iterate $o$ is found and is noted $\mathcal{J}^o$.
    \item Update $\Delta \bm{\phi}^{n,o}$ with the current set of positive Lagrange multiplier ($\mathcal{J}_o$) as per Equation \eqref{eq::updated_point}, \ie using:
    \begin{align}
        \Delta \bm{\phi}^{n,o+1} = \Delta\bm{\Tilde{\phi}}^n+ \sum_{j \in J^o} y_j \dd{f_j(\bm{\phi}^n)}{\bm{\phi}^n}.
    \end{align} 
    \item If, during steps 3 to 6, a constraint was either added or removed from the active set, go back to step 3 with the newly obtained $\Delta \bm{\phi}^{n,o+1}$; otherwise, exit the algorithm and use $\Delta \bm{\phi}^n=\Delta \bm{\phi}^{n,o+1}$ as the solution of the projection.
\end{enumerate}
\begin{figure}[!htpb]
	\centering
	\includegraphics[width=1\textwidth]{doc/active_set_workflow.pdf}
	\caption{Active set flowchart diagram.}
\label{fig::active_set_flowchart}
\end{figure}

To facilitate the understanding, Figure \ref{fig::active_set_flowchart} presents the workflow of the active set algorithm. This algorithm provides a projection of the point $\bm{\tilde{\phi}}^{n+1}$ onto the feasible set $\mathcal{Q}$ that minimizes Equation \eqref{eq::min_update}. This addition of constraint in bulk can lead to an overconstrained system. For this reason, the negative Lagrange multipliers are removed from the update. However, adding and subsequently removing multiple constraints from the active set can lead to oscillation, where constraints are repeatedly included and excluded from the active set. To mitigate oscillation and ensure convergence, the Lagrange multipliers are reevaluated using only the constraints with positive Lagrange multiplier values \cite{wong2011active} (loop between steps 5 and 6). The remainder of the section demonstrates the convergence of this modified algorithm.

To the authors' knowledge, the convergence of this algorithm has never been demonstrated. As such, the remainder of this section will show that this algorithm converges to a stable active set that respects the KKT criteria. First, let us introduce the KKT criteria for the point projection problem from Equations \eqref{eq::min_update}, \eqref{eq::eq_constraints_on_update}, and \eqref{eq::ineq_constraints_on_update}. Let $\mathcal{L^*}(\bm{\phi}^n)$ denote the Lagrangian of the projection problem, then optimality conditions are:

\begin{align}
    \dd {\mathcal{L^*}(\bm{\phi}^n)}{\bm{\phi}^n} &= (\Delta \bm{\phi}^n- \Delta\bm{\Tilde{\phi}}^n)  + \sum_{j\in J} y_j \dd {f_j(\bm{\phi}^n)}{\bm{\phi}^n} = \bm{0}, \label{eq::lagrangien_gradient_proj} \\
     f_j-\Delta \bm{\phi}^n \cdot \dd{f_j}{\bm{\phi}^n}  &= a_j \text{ for } j=0,1,2, \ldots, l, \\
     f_j-\Delta \bm{\phi}^n \cdot \dd{f_j}{\bm{\phi}^n}  &\leq a_j \text{ for } j=l+1, l+2, \ldots, m, \\
    y_j &\geq 0 \text{ for } j=l+1, l+2, \ldots, m.
    \label{eq::dual_feasibility}
    \\
    (f_j - a_j) y_j &= 0 \text{ for } j=l+1, l+2, \ldots, m.
    \label{eq::complementary_slackness}
\end{align}

To show the convergence of the proposed active set algorithm, the proof will demonstrate that the active set will be more constraining at each iteration than at the previous iteration ($\Vert \Delta\tilde{\bm{\phi}}^{n} - \Delta\bm{\phi}^{n,o+1} \Vert \leq \Vert \Delta\tilde{\bm{\phi}}^{n} - \Delta\bm{\phi}^{n,o+2} \Vert$), increasing the cost function while ensuring that the active set is self-compatible. This will ensure that all constraints are satisfied and that all of the KKT criteria are met at convergence, assuming that all constraints within the active set are linearly independent and that $\mathcal{Q}$ is feasible.

A set of constraints is considered self-compatible if the projection of $\Delta\tilde{\bm{\phi}}^{n}$ on it satisfies all the KKT criteria associated with this set, meaning that all constraints in this set are satisfied and inequality constraints have positive Lagrange multipliers. Let $ \tilde{\mathcal{J}}^o $ denote the active set after step 3 of iteration $ o $, corresponding to the current iterate $ \Delta\bm{\phi}^{n,o} $. Applying steps 5 and 6 removes the constraints in $ \tilde{\mathcal{J}}^o $ with negative Lagrange multipliers, resulting in a reduced set $ \mathcal{J}^o $ containing only positive Lagrange multipliers. 
By construction, $\mathcal{J}^o$ is thus self-compatible. The projection of $\Delta\tilde{\bm{\phi}}^n $ on this set results in iterate $\Delta\bm{\phi}^{n,o+1} $, which will be used in the next iteration. From this new point, the active set $ \tilde{\mathcal{J}}^{o+1} $ is constructed. Note that, by definition, $ \mathcal{J}^o \subseteq \tilde{\mathcal{J}}^{o+1}$. This new set is then subject to the same algorithm, leading to a reduced set $ \mathcal{J}^{o+1}$ from which $\Delta\bm{\phi}^{n,o+2}$ will be evaluated.
At the end of this process, three possible cases exist:

\begin{enumerate}
    \item \textbf{$ \mathcal{J}^o = \mathcal{J}^{o+1} $}: This equality implies that the projection on $ \mathcal{J}^o $ had already satisfied all KKT conditions of the projection problem (Equations \eqref{eq::lagrangien_gradient_proj} to \eqref{eq::complementary_slackness}). No further updates of the active set are necessary. 
    \item \textbf{$ \mathcal{J}^o \subset \mathcal{J}^{o+1} $}: In this case, new constraints are added alongside $ \mathcal{J}^o $, resulting in a projection onto $ \mathcal{J}^{o+1}$, which gives a more constrained solution. This implies through Pythagorean inequality that:
    \begin{align}
       \Vert \Delta\tilde{\bm{\phi}}^n - \Delta\bm{\phi}^{n,o+1} \Vert \leq \Vert \Delta\tilde{\bm{\phi}}^n - \Delta\bm{\phi}^{n,o+2} \Vert. 
       \label{eq::cost_increase_1}
    \end{align}
    \item \textbf{$ \mathcal{J}^o \not\subset \mathcal{J}^{o+1} $}: Since $ \mathcal{J}^{o+1} $ is obtained by first removing constraints with negative Lagrange multipliers from $ \tilde{\mathcal{J}}^{o+1} \setminus\mathcal{J}^{o}$, resulting in a set where the only constraints with a negative Lagrange multiplier are in $\mathcal{J}^{o}$, a self-compatible set. As it will be demonstrated in Lemma \ref{lemma::active_set_1} it implies that $\mathcal{J}^{o}$ is still satisfied by the projection on $\mathcal{J}^{o+1}$, and thus through Pythagorean inequality it means that:
    \begin{align}
       \Vert \Delta\tilde{\bm{\phi}}^n - \Delta\bm{\phi}^{n,o+1} \Vert \leq \Vert \Delta\tilde{\bm{\phi}}^n - \Delta\bm{\phi}^{n,o+2} \Vert. 
       \label{eq::cost_increase_2}
    \end{align}
\end{enumerate}
The validity of the third case relies on ensuring that removing constraints in $\mathcal{J}^{o}$ with negative Lagrange multipliers preserves the feasibility of these constraints. To formally prove this, we now introduce the following lemma:

\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}[section]  % Defines 

\begin{lemma}
Let $ \tilde{\mathcal{J}} $ be a set of constraints that contains a self-compatible subset $ \mathcal{J}$, meaning $ \mathcal{J} \subseteq \tilde{\mathcal{J}} $. Suppose the projection onto $ \tilde{\mathcal{J}} $ results in negative Lagrange multipliers for some of the inequality constraints in $ \mathcal{J} $, while all inequality constraints in $ \tilde{\mathcal{J}} \setminus \mathcal{J} $ have positive Lagrange multipliers. Then, removing all constraints with negative Lagrange multipliers from $ \tilde{\mathcal{J}} $ and projecting onto the reduced set, denoted $ \tilde{\mathcal{J}}_r $, ensures that all constraints in $ \mathcal{J} $ remain satisfied.
\label{lemma::active_set_1}
\end{lemma}
\begin{proof}
Let $ \tilde{\mathcal{J}} $ be a set of constraints containing a self-compatible subset $ \mathcal{J} \subseteq \tilde{\mathcal{J}} $. Suppose the projection onto $ \tilde{\mathcal{J}}$ results in negative Lagrange multipliers for some inequality constraints in $ \mathcal{J} $, forming a subset $ \mathcal{J}_- \subseteq \mathcal{J} $, while all inequality constraints in $ \tilde{\mathcal{J}} \setminus \mathcal{J} $ have positive Lagrange multipliers.

By dual feasibility and complementary slackness (fourth and fifth conditions of the KKT criteria, \ie Equations \eqref{eq::dual_feasibility} and \eqref{eq::complementary_slackness}), the constraints in $ \mathcal{J}_- $ should be inactive at the solution $ \Delta \bm{\phi}^n $, meaning $ f_j-\Delta \bm{\phi}^n \cdot \dd{f_j}{\bm{\phi}^n} < a_j $ for all $ j \in \mathcal{J}_- $ at the optimal solution. Since the inequality constraints in $ \tilde{\mathcal{J}} \setminus \mathcal{J} $ have no negative Lagrange multipliers, this movement inward cannot be caused by trying to satisfy any inequality constraints with negative Lagrange multipliers.

As $ \mathcal{J} $ is self-compatible, the constraints in $ \mathcal{J}_- $ have non-negative Lagrange multipliers when projected onto $ \mathcal{J} $ alone. This implies that the negative Lagrange multipliers are caused by interaction with $ \mathcal{J}^* \setminus \mathcal{J} $, and not by any internal conflict within $ \mathcal{J}_- $. This indicates that the optimal movement direction to minimize the cost function is driven by the active constraints in $ \tilde{\mathcal{J}} \setminus \mathcal{J} $, which pushes the solution away from the boundary defined by $ \mathcal{J}_- $. Therefore, the removal of all constraints in $ \mathcal{J}_- $ simultaneously does not break the feasibility of these constraints, as their inactive status is ensured by the external constraints in $ \tilde{\mathcal{J}}\setminus \mathcal{J} $.

Thus, projecting onto the reduced set $ \tilde{\mathcal{J}}_r = \tilde{\mathcal{J}} \setminus \mathcal{J}_- $ ensures that all constraints in $ \mathcal{J} $, including those in $ \mathcal{J}_- $, remain satisfied.
\end{proof}

This implies that in all three cases $\mathcal{J}^o= \mathcal{J}^{o+1}$, $\mathcal{J}^o \subset \mathcal{J}^{o+1}$, and $\mathcal{J}^o \not\subset \mathcal{J}^{o+1}$, the set used in the projection is self-compatible while also ensuring an increase in the cost function (Equations \eqref{eq::cost_increase_1}, and \eqref{eq::cost_increase_2}), guaranteeing the monotonicity of the algorithm's progress. It is important to note that while the iterates move further from the optimal solution at each iteration due to the addition of new constraints, this is done in a way that ensures the resulting active set is always compatible with itself. This process continues until no further constraints are violated, at which point the algorithm stops, leaving a final set that is both self-compatible and respects all constraints, satisfying the KKT criteria of the projection step \eqref{eq::lagrangien_gradient_proj}.







%%%%%%%%%%%%%%%%%%5 Wrong lemma %%%%%%%%%%%%%%%%%%%%

\begin{lemma}
Let $\mathcal{J}^o$ be a self-compatible active set. Let $\tilde{\mathcal{J}}^o$ be the set before the removal of constraints with negative Lagrange multipliers that led to the self-compatible set  $\mathcal{J}^o$ and let $\tilde{\mathcal{J}}^{o+1} \setminus \mathcal{J}^o$ be the subset of constraints from $\tilde{\mathcal{J}}^o \setminus \mathcal{J}^o$ that are reintroduced into the active set in the next iteration. Then, reintroducing $\tilde{\mathcal{J}}^{o+1} \setminus \mathcal{J}^o$ into $\mathcal{J}^o$ does not render any constraints in $\mathcal{J}^o$ redundant implying $\mathcal{J}^{o}\subset\mathcal{J}^{o+1}$.
\label{lemma::active_set_type1}
\end{lemma}

\begin{proof}
At iteration, $o$, $\mathcal{J}^o$ is a self-compatible active set that forms the boundary of the current solution.

Let $\tilde{\mathcal{J}}^o$ be the set that includes $\mathcal{J}^o$ and additional constraints that were removed due to negative Lagrange multipliers, forming $\tilde{\mathcal{J}}^o = \mathcal{J}^o \cup \mathcal{J}_-$, where $\mathcal{J}_-$ represents the set of constraints removed due to negative multipliers.

In the subsequent iteration, a subset $\tilde{\mathcal{J}}^{o+1} \setminus \mathcal{J}^o$ of previously removed constraints is reintroduced. These constraints were initially non-binding (with negative multipliers) but are reintroduced because they have become broken at the optimal point projection on the self-compatible set $\mathcal{J}^o$. This reintroduction indicates that these constraints were made redundant at the previous iteration due to interactions with other constraints with negative Lagrange multipliers.

Reintroducing $\tilde{\mathcal{J}}^{o+1} \setminus \mathcal{J}^o$ adds new boundaries to the region defined by the combined active set $\mathcal{J}^o \cup (\tilde{\mathcal{J}}^{o+1} \setminus \mathcal{J}^o)$. A constraint in $\mathcal{J}^o$ would only become redundant if the newly introduced constraints altered the feasible region such that some constraints in $\mathcal{J}^o$ no longer needed to be active.

However, since $\mathcal{J}^o$ was previously evaluated with $\tilde{\mathcal{J}}^o$, none of its constraints were redundant as all had positive multipliers. The reintroduction of $\tilde{\mathcal{J}}^{o+1} \setminus \mathcal{J}^o$ only adds constraints that became binding due to the removal of other constraints with negative Lagrange multipliers. Since all constraints in $\mathcal{J}^o$ were binding with positive Lagrange multipliers in a more restricted feasible region (the space defined by $\tilde{\mathcal{J}}^o$) compared to the feasible region defined by $\tilde{\mathcal{J}}^{o+1}$, which includes the reintroduced constraints $\tilde{\mathcal{J}}^{o+1} \setminus \mathcal{J}^o$, these newly binding constraints cannot make the constraints in $\mathcal{J}^o$ redundant, this follows from the fact that $\tilde{\mathcal{J}}^{o+1}$ is formed from a subset of $\tilde{\mathcal{J}}^o$, ensuring that $\mathcal{J}^o$ remains necessary for maintaining their feasibility and non-redundancy.

Therefore, reintroducing $\tilde{\mathcal{J}}^{o+1} \setminus \mathcal{J}^o$ ensures that the active set $\mathcal{J}^o$ continues to have positive Lagrange multipliers with no constraints in $\mathcal{J}^o$ becoming redundant.
\end{proof}

==> src/convergence_demo.tex <==
Assuming that the gradient of the cost function is Lipschitz continuous the following inequality holds:

 \begin{equation}
    \begin{split}
    \mathcal{C}(\bm{\phi^{n+1}})\leq &\mathcal{C}(\bm{\phi^{n}})- \dd {\mathcal{C}(\bm{\phi}^n)}{\bm{\phi}^n} \cdot ( \min(1,\frac{\gamma^n}{\alpha^n})\Delta\bm{\phi^{n}}_\parallel +\frac{\gamma^n}{\alpha^n}\Delta\bm{\phi^{n}}_\perp)\\ &+\frac{L}{2} \left\Vert- \min(1,\frac{\gamma^n}{\alpha^n})\Delta\bm{\phi^{n}}_\parallel-\frac{\gamma^n}{\alpha^n}\Delta\bm{\phi^{n}}_\perp\right\Vert^2
    \end{split}
\end{equation}

Here, $L$ is the Lipschitz constant of the gradient of the cost function. From this, to have $\mathcal{C}(\bm{\phi^{n+1}})\leq \mathcal{C}(\bm{\phi^{n}})$ holds the following inequation must also be true:

 \begin{equation}
    \begin{split}
     -\dd {\mathcal{C}(\bm{\phi}^n)}{\bm{\phi}^n} \cdot \left(\min(1,\frac{\gamma^n}{\alpha^n})\Delta\bm{\phi^{n}}_\parallel +\frac{\gamma^n}{\alpha^n}\Delta\bm{\phi^{n}}_\perp\right) +\frac{L}{2} \left\Vert-\Delta\bm{\phi^{n}}_\parallel-\frac{\gamma^n}{\alpha^n}\Delta\bm{\phi^{n}}_\perp\right\Vert^2 \leq 0 
    \end{split}
\end{equation}

Substituting $\Delta\bm{\phi^{n}}_\parallel$ and $\Delta\bm{\phi^{n}}_\perp$ by their definition as projections on two orthogonal subspaces,

 \begin{align}
 \Delta\bm{\phi^{n}}_\parallel&=\lambda_\parallel \left(\alpha^n  \dd {\mathcal{C}(\bm{\phi}^n)}{\bm{\phi}^n}_\parallel -\beta^n(\bm{\phi}^n-\bm{\phi}^{n-1})_\parallel\right)\\
 \Delta\bm{\phi^{n}}_\perp&=\lambda_\perp\left(\alpha^n  \dd {\mathcal{C}(\bm{\phi}^n)}{\bm{\phi}^n}_\perp-\beta^n(\bm{\phi}^n-\bm{\phi}^{n-1})_\perp\right)
 \end{align}
where $\lambda_\parallel$ and $\lambda_\perp$ are real constants between 0 and 1.
  \begin{equation}
    \begin{split}
- \lambda_\parallel\min\left(1,\frac{\gamma^n}{\alpha^n}\right)\dd {\mathcal{C}(\bm{\phi}^n)}{\bm{\phi}^n} \cdot\left(\alpha^n   \dd {\mathcal{C}(\bm{\phi}^n)}{\bm{\phi}^n}_\parallel -\beta^n(\bm{\phi}^n-\bm{\phi}^{n-1})_\parallel\right)\\ 
     -\frac{\gamma^n\lambda_\perp}{\alpha^n} \dd {\mathcal{C}(\bm{\phi}^n)}{\bm{\phi}^n} \cdot \left(\alpha^n  \dd {\mathcal{C}(\bm{\phi}^n)}{\bm{\phi}^n}_\perp-\beta^n(\bm{\phi}^n-\bm{\phi}^{n-1})_\perp \right) \\+\frac{L}{2} \left\Vert-\lambda_\parallel\min\left(1,\frac{\gamma^n}{\alpha^n}\right)\left(\alpha^n  \dd {\mathcal{C}(\bm{\phi}^n)}{\bm{\phi}^n}_\parallel -\beta^n(\bm{\phi}^n-\bm{\phi}^{n-1})_\parallel\right)\right\Vert^2 \\+ \frac{L}{2} \left\Vert-\frac{\gamma^n\lambda_\perp}{\alpha^n}\left(\alpha^n  \dd {\mathcal{C}(\bm{\phi}^n)}{\bm{\phi}^n}_\perp-\beta^n(\bm{\phi}^n-\bm{\phi}^{n-1})_\perp\right)\right\Vert^2 \leq 0 
    \end{split}
\end{equation}

Regrouping terms give the following inequality:
\begin{equation}
    \begin{split}
\left( -\alpha^n \lambda_\parallel\min\left(1,\frac{\gamma^n}{\alpha^n}\right)  + 0.5 {\alpha^n}^2 L \lambda_\parallel^2 \min\left(1,\frac{\gamma^n}{\alpha^n}\right)^2\right) \left\Vert\dd {\mathcal{C}(\bm{\phi}^n)}{\bm{\phi}^n}_\parallel \right\Vert^2 \\+   \left( -\gamma^n \lambda_\perp  + 0.5 {\gamma^n}^2 L \lambda_\perp^2 \right)\left\Vert\dd {\mathcal{C}(\bm{\phi}^n)}{\bm{\phi}^n}_\perp \right\Vert^2  \\+\beta^n\left(  \lambda_\parallel\min\left(1,\frac{\gamma^n}{\alpha^n}\right)-\alpha^n L \lambda_\parallel^2\min\left(1,\frac{\gamma^n}{\alpha^n}\right)^2\right)\dd {\mathcal{C}(\bm{\phi}^n)}{\bm{\phi}^n}_\parallel \cdot (\bm{\phi}^n-\bm{\phi}^{n-1})_\parallel\\+\beta^n\left(\lambda_\perp \frac{\gamma^n}{\alpha^n}-\alpha^n  L \lambda_\perp^2\left(\frac{\gamma^n}{\alpha^n}\right)^2\right)\dd {\mathcal{C}(\bm{\phi}^n)}{\bm{\phi}^n}_\perp \cdot (\bm{\phi}^n-\bm{\phi}^{n-1})_\perp\\+  0.5 {\beta^n}^2 L \lambda_\parallel^2\min\left(1,\frac{\gamma^n}{\alpha^n}\right)^2\left\Vert (\bm{\phi}^n-\bm{\phi}^{n-1})_\parallel \right\Vert^2\\+0.5  {\beta^n}^2 L \lambda_\perp^2\left(\frac{\gamma^n}{\alpha^n}\right)^2 \left\Vert (\bm{\phi}^n-\bm{\phi}^{n-1})_\perp \right\Vert^2\leq 0
\label{eq::developped_convergence_regroup_terms}
    \end{split}
\end{equation}

Three sufficient conditions are generated from Equation \eqref{eq::developped_convergence_regroup_terms} to guarantee the inequality. 

 \begin{align}
    \lambda_\parallel \alpha^n\min(1,\frac{\gamma^n}{\alpha^n})&\leq\frac{2}{L}
   \label{eq::constraint_on_alpha}&\\
    \lambda_\perp\gamma^n&\leq\frac{2}{L}&
    \label{eq::constraint_on_gamma}\\
    \begin{split}
    \vert \beta^n\left(  \lambda_\parallel\min\left(1,\frac{\gamma^n}{\alpha^n}\right)-\alpha^n L \lambda_\parallel^2\min\left(1,\frac{\gamma^n}{\alpha^n}\right)^2\right)\dd {\mathcal{C}(\bm{\phi}^n)}{\bm{\phi}^n}_\parallel \cdot (\bm{\phi}^n-\bm{\phi}^{n-1})_\parallel\\+\beta^n\left(\lambda_\perp \frac{\gamma^n}{\alpha^n}-\alpha^n  L \lambda_\perp^2\left(\frac{\gamma^n}{\alpha^n}\right)^2\right)\dd {\mathcal{C}(\bm{\phi}^n)}{\bm{\phi}^n}_\perp \cdot (\bm{\phi}^n-\bm{\phi}^{n-1})_\perp\\+  0.5 {\beta^n}^2 L \lambda_\parallel^2\min\left(1,\frac{\gamma^n}{\alpha^n}\right)^2\left\Vert (\bm{\phi}^n-\bm{\phi}^{n-1})_\parallel \right\Vert^2\\+0.5  {\beta^n}^2 L \lambda_\perp^2\left(\frac{\gamma^n}{\alpha^n}\right)^2 \left\Vert (\bm{\phi}^n-\bm{\phi}^{n-1})_\perp \right\Vert^2\vert\\ \leq\vert \left( -\alpha^n \lambda_\parallel\min\left(1,\frac{\gamma^n}{\alpha^n}\right)  + 0.5 {\alpha^n}^2 L \lambda_\parallel^2 \min\left(1,\frac{\gamma^n}{\alpha^n}\right)^2\right) \left\Vert\dd {\mathcal{C}(\bm{\phi}^n)}{\bm{\phi}^n}_\parallel \right\Vert^2 \\+   \left( -\gamma^n \lambda_\perp  + 0.5 {\gamma^n}^2 L \lambda_\perp^2 \right)\left\Vert\dd {\mathcal{C}(\bm{\phi}^n)}{\bm{\phi}^n}_\perp \right\Vert^2 \vert&
    \label{eq::constraint_inertia}
    \end{split}
\end{align}
The first two (Inequation \eqref{eq::constraint_on_alpha}and \eqref{eq::constraint_on_gamma}) ensure that optimization is converging, and the third Inequation (\eqref{eq::constraint_inertia}) ensures that the variation of the solution due to the presence of inertia is smaller than the contribution of the gradient descent. Taking the coefficient $\lambda_\parallel=1$, $\lambda_\perp=1$, and the terms $\min\left(1,\frac{\gamma^n}{\alpha^n}\right)=1$ as they are the most constraining values for the size of the step $\alpha$ and $\gamma$, Inequations \eqref{eq::constraint_on_alpha}and \eqref{eq::constraint_on_gamma}simplify to:
 
\begin{align}
    \begin{split}
    \gamma^n\leq\frac{2}{L}
    \label{eq::constraint_gamma_final}
    \end{split}
\end{align}

Inequation can be hard to evaluate; as such, a good estimate of the bounds of $\beta$ can be obtained by simplifying this inequation by assuming that the active set of constraints is empty, meaning $\lambda_\parallel=1$ and  $\lambda_\perp=1$. Then, the largest bounds on $\beta^n$ can be found by maximizing the righthand side of the equation by taking and $\alpha^n=\gamma^n=\frac{1}{L}$. Applying these assumptions reduces the Inequation \eqref{eq::constraint_inertia} to: 
\begin{align}
    \begin{split}
{\beta^n}\leq \frac{1}{L} \frac{ \left\Vert\dd {\mathcal{C}(\bm{\phi}^n)}{\bm{\phi}^n}\right\Vert }{\left\Vert (\bm{\phi}^n-\bm{\phi}^{n-1}) \right\Vert}
    \label{eq::inertia_final_bounds}
    \end{split}
\end{align}
These bounds do not guarantee convergence without using $\alpha^n=\gamma^n=\frac{1}{L}$. Note here that $\gamma^n$ is defined using an estimation of the Lagrangian gradient, which is evaluated after the projection. This means that in practice, $\gamma^n \neq \alpha^n$. However, they are generally relatively close since the gradient of the Lagrangian is generally mostly controlled by the gradient of the cost function. Additionally, a good estimate of $L$ is required to use these bounds to define the parameter. A Generally good local estimate of $L$ can be obtained by taking 
$L=\frac{}{}$

Based on this analysis, the following choices of steps are made: 

\begin{align}
    \begin{split}
\alpha=\frac{1}{L}
    \label{eq::constraint_first_simplification }
    \end{split}
\end{align}

\begin{align}
    \begin{split}
{\beta^n}\leq \frac{1}{L} \frac{ \left\Vert\dd {\mathcal{C}(\bm{\phi}^n)}{\bm{\phi}^n}\right\Vert }{\left\Vert (\bm{\phi}^n-\bm{\phi}^{n-1}) \right\Vert}
    \label{eq::constraint_first_simplification }
    \end{split}
\end{align}





\begin{comment}
\begin{equation}
    \begin{split}
\max\left(\left( -\alpha^n \lambda_\parallel\min\left(1,\frac{\gamma^n}{\alpha^n}\right)  + 0.5 {\alpha^n}^2 L \lambda_\parallel^2 \min\left(1,\frac{\gamma^n}{\alpha^n}\right)^2\right), \left( -\gamma^n \lambda_\perp  + 0.5 {\gamma^n}^2 L \lambda_\perp^2 \right)\right)\\\left\Vert\dd {\mathcal{C}(\bm{\phi}^n)}{\bm{\phi}^n} \right\Vert^2 \\+
\beta^n\max\left(
\left(  \lambda_\parallel\min\left(1,\frac{\gamma^n}{\alpha^n}\right)-\alpha^n L \lambda_\parallel^2\min\left(1,\frac{\gamma^n}{\alpha^n}\right)^2\right), \left(\lambda_\perp \frac{\gamma^n}{\alpha^n}-\alpha^n  L \lambda_\perp^2\left(\frac{\gamma^n}{\alpha^n}\right)^2\right)\right)
\\ \left\Vert\dd {\mathcal{C}(\bm{\phi}^n)}{\bm{\phi}^n}\right\Vert \left\Vert (\bm{\phi}^n-\bm{\phi}^{n-1})\right\Vert \\+ {\beta^n}^2 0.5  L \max\left(
 \lambda_\parallel^2\min\left(1,\frac{\gamma^n}{\alpha^n}\right)^2,  \lambda_\perp^2\left(\frac{\gamma^n}{\alpha^n}\right)^2\right)\left\Vert (\bm{\phi}^n-\bm{\phi}^{n-1}) \right\Vert^2
\leq 0
\label{eq::developped_convergence_regroup_terms}
    \end{split}
\end{equation}



\begin{equation}
    \begin{split}
\left( -\alpha^n \lambda_\parallel\min\left(1,\frac{\gamma^n}{\alpha^n}\right)  + 0.5 {\alpha^n}^2 L \lambda_\parallel^2 \min\left(1,\frac{\gamma^n}{\alpha^n}\right)^2\right) \left\Vert\dd {\mathcal{C}(\bm{\phi}^n)}{\bm{\phi}^n}_\parallel \right\Vert^2 \\+   
\left( -\gamma^n \lambda_\perp  + 0.5 {\gamma^n}^2 L \lambda_\perp^2 \right)
\left\Vert\dd {\mathcal{C}(\bm{\phi}^n)}{\bm{\phi}^n}_\perp \right\Vert^2  \\+
\beta^n\left(  \lambda_\parallel\min\left(1,\frac{\gamma^n}{\alpha^n}\right)-\alpha^n L \lambda_\parallel^2\min\left(1,\frac{\gamma^n}{\alpha^n}\right)^2\right)
\dd {\mathcal{C}(\bm{\phi}^n)}{\bm{\phi}^n}_\parallel \cdot (\bm{\phi}^n-\bm{\phi}^{n-1})_\parallel\\+
\beta^n\left(\lambda_\perp \frac{\gamma^n}{\alpha^n}-\alpha^n  L \lambda_\perp^2\left(\frac{\gamma^n}{\alpha^n}\right)^2\right)
\dd {\mathcal{C}(\bm{\phi}^n)}{\bm{\phi}^n}_\perp \cdot (\bm{\phi}^n-\bm{\phi}^{n-1})_\perp\\+  
0.5 {\beta^n}^2 L \lambda_\parallel^2\min\left(1,\frac{\gamma^n}{\alpha^n}\right)^2\left\Vert (\bm{\phi}^n-\bm{\phi}^{n-1})_\parallel \right\Vert^2\\+
0.5  {\beta^n}^2 L \lambda_\perp^2\left(\frac{\gamma^n}{\alpha^n}\right)^2 \left\Vert (\bm{\phi}^n-\bm{\phi}^{n-1})_\perp \right\Vert^2
\leq 0
\label{eq::developped_convergence_regroup_terms}
    \end{split}
\end{equation}

\end{comment}




